EchoNarrator: Generating natural text explanations for ejection fraction predictions

Ejection fraction (EF) of the left ventricle (LV) is considered as one of the most important measurements for diagnosing acute heart failure and can be estimated during cardiac ultrasound acquisition. While recent successes in deep learning research successfully estimate EF values, the proposed models often lack an explanation for the prediction. However, providing clear and intuitive explanations for clinical measurement predictions would increase the trust of cardiologists in these models. In this paper, we explore predicting EF measurements with Natural Language Explanation (NLE). We propose a model that in a single forward pass combines estimation of the LV contour over multiple frames, together with a set of modules and routines for computing various motion and shape attributes that are associated with ejection fraction. It then feeds the attributes into a large language model to generate text that helps to explain the network's outcome in a human-like manner. We provide experimental evaluation of our explanatory output, as well as EF prediction, and show that our model can provide EF comparable to state-of-the-art together with meaningful and accurate natural language explanation to the prediction. The project page can be found at https://github.com/guybenyosef/EchoNarrator .

==> sections/discussion.tex <==
% \begin{itemize}
%     \item limitations: dataset size, noise in pseudo labels and data quality
%     \item lessons learned: metrics, model size, self instruct
% \end{itemize}

%This analysis underscores the value of synthetic data augmentation in overcoming the limitations of small datasets, a common challenge in the medical domain. By effectively leveraging large language models and synthetic augmentation, we demonstrate that it is possible to significantly enhance the quality of explanations without compromising on the accuracy of EF predictions. 


Our model introduces an innovative approach to EF prediction and NLE generation, leveraging a GCN coupled with the LLaMA model for end-to-end inference. Despite demonstrating notable successes, we acknowledge limitations such as the constrained size of the dataset, the presence of noise in keypoints and prompts, and varying data quality, which could impact the robustness and generalizability of our findings. The use of another LLM to evaluate the performance of the approach turned out to be most informative and sensitive towards contradictions. However, LLM-based evaluation highly depends on the chosen configuration and prompt design which influences sensibility and variability. Incorporating additional human-based evaluation will be necessary in the future. 
%The value of synthetic data increase to mitigate the challenges posed by limited datasets.
Through the strategic use of synthetic data, data augmentation and LLMs, we have shown that it is feasible to improve interpretability of EF predictions without sacrificing accuracy. This balance is essential for the broader clinical adoption of AI, where clear and understandable explanations are as crucial as the predictions. 

==> sections/exp.tex <==
\subsection{Data}
\label{sec:data}
{\bf Dataset.} We use the EchoNet-Dynamic dataset~\cite{ouyang2020video}, which contains 10,030 echocardiography videos from healthy and pathological patients. Each video is annotated with 40 LV contour points, one basal and apex point at the end-diastolic (ED) and end-systolic (ES) frame, along with the EF. The dataset is divided into $80\%$ training, $10\%$ validation and $10\%$ testing splits. 

% The pipeline was trained and evaluated in the public EchoNet dataset \cite{Ouyang} with 10,030 echocardiography videos of healthy and pathological patients. All videos have one ED and one ES frame for a selected cycle labeled with 40 annotated keypoints representing the LV contour plus two additional keypoints for the basal and apex points. Furthermore, the dataset provides EF values for each sequence. The publicly available splits are $80\%$ training, $10\%$ validation, and $10\%$ test sets for direct comparison. For each dataset we identified the ED and ES frames and sampled 14 additional intermediate frames evenly spaced, to reduce the computation complexity.

% \subsection{Annotations}
% \label{sec:annotations}
%\todo{[Sarina] -- here to describe the processing of acquiring annotations for the EF explanation, including the data set from whit they were taken, the procedure, the acquiring and transcript process with model (e.g., Whisper v3), the vlaidation with clinical experts, and the cleaning you did manually}

{\bf Annotations.} 
We trained our GCN models on the annotated keypoints from the EchoNet dataset, employing a multi-frame strategy in~\cite{ours2022miccai}. To simplify the processing, we selected ED and ES frames and sampled 14 evenly spaced intermediate frames from each video.
A lack of Electronic Health Records (EHR) text data from EchoNet dataset prompting us to enlist two cardiology experts who annotate a subset of the training data with video-text pairs. 
The experts watched the videos and provided descriptions including their EF assessments and reasoning, focusing on attributes like LV shape, wall movement, and bulge presence. Experts were allowed to use different structures or formats in their descriptions  which ensures a diverse text reflection of real-world scenarios. 89 image-text pairs were generated for training, with additional 48 pairs designated for testing. 
% Acquiring EHR data paired with ultrasound data is highly restrictive and the experiments were solely based on the public dataset EchoNet \cite{ouyang2020video} that comes with EF values and two annotated keyframes with keypoints contouring the LV. The GCN models were trained on the keypoints following the multi-frame approach in \cite{ours2022miccai}. \todo{specify} EchoNet does not include any EHR text data. Two cardiology experts were asked to label a subset of the training data. They were shown each video and asked to describe the video by focusing on the left ventricle in particular and answering the question on how they would rate the EF and why. They further got the instruction to think about some key attributes associated with the EF like the shape, wall movement, and bulge. However, experts were not restricted in their answers to create a highly variable real-world dataset. In total they created a dataset with 89 image-text pairs for training and \todo{XX} image-text pairs for testing. Given the already annotated keypoints, several attributes were calculated to generate an input for the LLM.

\subsection{NLE evaluation metrics}
\label{sec:metrics}
We incorporated several different evaluation metrics to evaluate our LLM outputs from different aspects utilizing the advantages of each.
% We exploit the \textbf{BERT} score \cite{zhang2019bertscore} which compares sentences based on cosine similarity of their embeddings,  \textbf{BioBERT}~\cite{lee2020biobert} and \textbf{ClinicalBERT}~\cite{huang2019clinicalbert} which are designed for clinical texts to improve relevance by capturing medical attributes. Considering their enhanced reasoning capabilities, we also experiment with Sentence-based BERT models (\textbf{sBERT}) \cite{reimers-2019-sentence-bert} which generate a single embedding per sentence, and \textbf{MedsBERT}~\cite{rasmy2021med} that pre-trained on clinical texts.
We exploit the \textbf{ClinicalBERT}~\cite{huang2019clinicalbert} and Sentence-based BERT models (\textbf{sBERT})~\cite{rasmy2021med} that generate single embeddings either per word and per sentence followed by cosine similarity and are pre-trained on clinical texts. Additional text similarity models are provided in the suppl. material.
% To address the critical issue of contradictions in clinical explanations overlooked by BERT scores, we incorporate \textbf{SimCSE} \cite{gao2021simcse}, a similarity metric based on contrastive learning to discern and handle contradictions.
The Mistral score was introduced to evaluate explanations against specific clinical attributes, leveraging a recently developed \textbf{Mistral LLM}~\cite{jiang2023mistral} tailored for this purpose. This custom metric (sec. \ref{subsec:methods:metric_ef_text}), aims to provide a more nuanced assessment of the clinical relevance and accuracy of the explanations generated. In addition to accuracy metrics, we also used the Flesch Reading Ease score to measure contextual richness of the explanation (a lower Flesch score means contextually richer text).  



% \todo{[Sarina] -- here we can mention the different metrics, and refer to the MIstarl metric described at the Method sec.. }
% \todo{Here is another paper that could be cited?}
% https://arxiv.org/html/2401.11505v1 they use chexbert.
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC9055736/ contrastive training of chexbert

% Tab. 1 - EF prediction
% EF, MKE

% Tab. 2 - NLE prediction 
% \newline
% {\bf NLP scores:} Often two classical NLP inspired scores are used in the literature, namely BLEU and ROUGE \todo{REF}. Both measure the overlap of ngrams (n words) between a generated sentence and a reference. BLEU measures precision, whereas ROUGE measures recall. The scores do not take into account any reasoning and are dependent on the input sequence length. Although widely reported, these scores are not well suited for critical tasks like clinical explanations.
% \newline
% {\bf BERT scores:}
% More sophisticated is the BERT score (BERT), which uses a trained language encoder to create embeddings of two sentences that are compared according to the cosine-similarity. There are many pre-trained variants of BERT (BioBERT, clinicalBERT)\todo{REF}, some also explicitly trained on clinical text. Using more targeted versions can help identify key medical attributes. However, BERT can still fail due to contradictions and factual errors. Compared to word-based BERT models, sentence-based BERT (sBERT) produce one embedding for each sentence that might help with the reasoning. Those models can also be pre-trained on clinical text (medsbert).
% \newline
% {\bf simcse}
% Since contradictions are very critical, a similarity metric is added that was designed to handle contradictions by contrastive learning \todo{REF}. 
% \newline
% {\bf mistral score}
% As described in sec. \ref{subsec:methods:metric_ef_text}, a customized metric was added to target specific attributes using a recently pre-trained mistral LLM. \todo{REF}\newline

% \todo{maybe mention Chexbert??}



%\begin{enumerate}
%    \item BERT similarity score
%%    \item medical-based BERT similarity scores
%   \item BERT sentence similarity score
%    \item medical-based BERT sentence similarity scores
%    \item NLP scores, BLEU, ROUGE
%    \item costum MISTRAL score - contradictions, ratio
%    \item richness of text
%\end{enumerate}



\subsection{EF predictions with generated explanations}
\label{sec:predictions}
{\bf Implementation:} Our GCN model uses a ResNet-3D-18 as video encoder backend, optimizing for the efficient processing of echocardiography videos. GCN model training focuses on accurately predicting LV keypoints, which are crucial for the subsequent estimation of EF and the generation of explanations. For the NLE component, we train the LLaMA model to generate clinically relevant explanations based on attributes derived from the GCN output. 
LLM training included a low-rank adaptation on the LLaMA-1 model through 8-bit quantization, with a learning rate of $0.0003$ and a batch size of 32. Training was performed for 5 hours on two A6000 GPUs, each equipped with 48GB memory. 
The end-to-end inference pipeline ensures a seamless transition from raw video data to EF predictions accompanied by understandable explanations. Detailed implementation specifics and source code are available on GitHub for reproducibility\footnote{https://github.com/xxx/xxx}.

{\bf Results:} In evaluating our end-to-end inference system, we focus on both, the EF prediction accuracy and the quality of the generated explanations. While competitors exist for EF prediction, our approach is unique in integrating NLE, setting a benchmark in the field. 
Tab.~\ref{tab:ef} lists the details of our comparison with previous models using the Dice score, mean keypoint error (MKE), and EF prediction accuracy. We show that our single task NLE GCN can reach lower MKE than the EchoGraph while maintaining the same EF accuracy. Predicting from volumes (Vol) versus predicting directly from keypoints (EF) performed similarly well.  
For NLE prediction, we evaluate the coherence and clinical relevance of the generated explanations quantitatively (Tab.~\ref{tab:nle}) and qualitatively (Fig.~\ref{fig:plots}). In Tab.~\ref{tab:nle}, we added a prediction of the LLaVA-Med model~\cite{li2024llava} when we input an image showing ED and ES frames, followed by the instruction to explain the EF (see suppl. material for details). Although different from our model in the design and goal, it seems to be the closest in providing baseline text explanations.
%

{\bf Analysis:} 
Our results demonstrate notable accuracy in EF prediction (Tab.~\ref{tab:ef}) combined with the generation of clinically meaningful explanations. Compared to competitors in EF predictions, the scores in Tab.~\ref{tab:nle} further show that our system not only achieves good EF estimation, but also introduces the capability of generating accurate, complete, and human-like explanations. Tab.~\ref{tab:nle} also shows that predicted explanations are better from simple baselines. 
%This advancement significantly improves the interpretability of EF predictions in clinical settings, bridging the gap between automated analysis and practical medical application.
%
%\todo{Here we should describe the effect of improvement in NLE (according to the metrics discussed above) with the increase of synthetic data and augmentations. }
The enhancement of NLE prediction in our model can be attributed to the use of synthetic data and data augmentation techniques (Sec.~\ref{subsec:methods:explanationgeneration}). 
% As evidenced by the metrics described in Tab.~\ref{tab:nle}, our approach shows a clear trend: Incorporating synthetic data, especially when scaled, improves the coherence and clinical relevance of the generated explanations. 
The utilization of the self-instruction by using Chain-of-Thought in GPT4 further refines the model's capability to generate plausible and contextually more rich explanations that meet clinical expectations, as shown by its lower scores in the Reading Ease metric.
% \todo{Do we have a metric to evaluate the contextual richness? We can then say that the pseudo-explanations might be as correct at the best LLAMA model, but LLAMA is much better in contextual richness}


% \todo{PART 1 for this subsection: here we should describe the implementation details for running the training of the GCN, and training of the LLaMA model, and the end-to-end inference. }

% The GCN is trained with a r3d\_18 video encoder backend. Further implementation details can be found the supplementary material and source code to reproduce the given results is on Github: \url{XXX}.
% \todo{not sure how many details for the LLM we can list here}

% \todo{PART 2 for this subsection: Here we should point to the results achieved for evenluating the end-to-end inference, and point to both the EF prediction result and the explanation results. We should say something about the comettitors -- there are only for the EF prediction, not for the NLE. We should point here to both the quantitative eval (the tables) and the qualitative eval (the Figure).  }

% \textbf{EF prediction:} We compare different extensions to previous work \cite{ours2022miccai}, in which the EF is either directly computed from the encoder, with the EF regressed from the kpts and the volumes. 
% %We compare to two semantic segmentation algorithms: the DeepLabv3 approach from EchoNet~\cite{Ouyang}  and the nnU-Net~\cite{isensee2021nnu}. 
% Results for several different models are shown in Tab.~\ref{tab:ef} where all approaches were compared on Dice score, mean keypoint error and EF. EchoNet does not have real image sizes so to calculate keypoint error, coordinates were normalized by image dimensions.

% \textbf{NLE prediction:}\newline

% \todo{PART 3 for this subsection: Here we should briefly summarize the results, say what is good, how are we compared to our compettitors, and how are we compared to baselines. }


% potential table 3
% \begin{enumerate}
%     \item human ?
% \end{enumerate}


\input{tables/table_ef}


% Experiments already run
% \begin{enumerate}
%     \item lORA 7 b 1 to 1
%     \item lORA 13 b 1 to 1
%     \item LORA self instruct
% \end{enumerate}

\input{tables/table_nle}
%\todo{maybe it is necessary to run the mistral 10 times for each to see whether the answers depend on stochastics?}
% Remark: I put the best result for the GPT version (we tested different examples)


%\subsection{Evaluation of the single task multi-frame model}

%\subsection{Evaluation of the text generation}
%\label{subsec:experiments:textgen}
%Clinical reports that describe properties of the LV with respect to the EF are not available and the public dataset only contains segmentation and EF. To examine whether the text generator outcome aligns with the image input and annotations, we compute a similarity score between annotations and text explanations. The keypoint annotations can be used to compute the Euclidean distance between two instances. For this purpose, both ED and ES frames must be registered first which can be done with least square approximation. In addition, the EF between two instances can be compared. 

%For the text similarity, the Siamese BERT (SBERT) model \cite{reimers-2019-sentence-bert} is utilized that uses siamese and triplet networks creating sentence embeddings for each of the provided sentences. The cosine-similarity between those embeddings serves as a metric for comparison.
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=1.\textwidth]{plot_correlation_distribution.png}
%    \caption{Left:This is the distribution of attributes computed from the multi-frame model which looks similar to the attributes computed from the single frame model. Right: Correlation plot between the sentence similarity and the EF similarity. It seems that we cannot correlate it with this metric maybe because there is too much other text and it works better if we integrate kpts similarity \todo{Add kpts similarity, This is only for you Qing, might be thrown out of the paper.}} 
%    \label{fig:plots}
%\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.97\textwidth]{figures/results_fig_new2.png}
    \caption{(Zoom in for optimal view) LV contour estimation, EF prediction and its text explanation as provided by the NLE-EF-13B self-instruct on EchoNet test examples.} %(Zoom in for optimal view.) 
    \label{fig:plots}
\end{figure}



==> sections/intro.tex <==
The release of the extensive Dynamic EchoNet echocardiography dataset~\cite{ouyang2020video} has accelerated the adoption of deep learning models for ejection fraction (EF) prediction and left ventricle (LV) contour delineation. Several innovative approaches have been introduced, including LV segmentation \cite{ouyang2020video,Weihang2023,Meng2024}, direct video regression \cite{ouyang2020video,kazemi2020deep,reynaud2021ultrasound,rand2022miccai}, graph- and keypoints-based models \cite{Mokhtari2022miccai,ours2022miccai}, and attention-based models \cite{Mokhtari2023} - Their potential is somewhat diminished by a common shortfall: the lack of clinically meaningful explanations for the predicted EF. %This gap between technological advancement and clinical applicability underscores a critical need for models that do more than just predict; they must also communicate their findings in a manner that aligns with clinical insight and understanding.
Explainability of visual deep learning models is often linked with activation maps such as Class Activation Mapping (CAM)~\cite{zhou2016learning} and Grad-CAM~\cite{selvaraju2017grad}, which associate image regions with their contribution to the prediction. Although useful in certain contexts, these methods often fall short in medical imaging, where they may only highlight obvious regions such as the LV to predict EF, providing clinically correct but not meaningful information (an interesting example of this phenomenon was shown in~\cite{Mokhtari2023}). To overcome these limitations and improve the explainability with human-like text, a novel approach has been developed within the subfield of {\em Natural Language Explanations} (NLE). This approach leverages advancements in vision-language and language models to generate text explanations that accompany model outcomes, providing context and clarity that activation maps cannot provide. NLE models include the generation of text explanations based on object attributes~\cite{hendricks2016generating}, models for associating text explanations with image regions~\cite{hendricks2018grounding}, and language models such as GPT2 \cite{sammani2022nlx,kayser2022explaining} and GPT3 \cite{sammani2023iccvw}. Considering that abnormal EF values are often linked to visible changes in the LV, providing explanations based on those visual cues shall enhance cardiologists' confidence in the deep learning predictions. 
Inspired by attribute-based NLE strategies (e.g., ~\cite{hendricks2016generating,hendricks2018grounding}), where explanations are generated based on a predefined set of attributes, we create attributes that influence EF predictions, such as wall thickening in the interventricular septum (hereafter referred to as bulge), regional wall motion abnormalities, and foreshortening due to acquisition. Furthermore, we incorporate Large Language Models (LLMs) into our pipeline, utilizing models like LLaMA~\cite{touvron2023llama} as the final step to synthesize smooth and coherent explanations. 
% The pre-trained model is enriched with medical knowledge to ensure that the generated text is accurate and clinically relevant.

Our innovation harnesses the capabilities of LLMs to assimilate the estimation of relevant LV attributes, generating text explanations that are informative and aligned with clinical practices. This method marks a significant step toward developing an AI assistant capable of engaging with clinicians through human-like language. %, enhancing the interpretability of EF predictions.
%Old
%The value of explainability in clinical measurement predictions cannot be overstated, particularly when it comes to estimating the ejection fraction (EF) of the heart using cardiac ultrasound. An explanation that resonates with the intuition of cardiologists is crucial, as it significantly increases their confidence in the prediction. Pathological variations of the EF are often attributed to observable changes in the left ventricle (LV). By putting explanations on these visual cues, we can not only promote increased confidence, but also diminish the need for time-consuming manual adjustments that currently impede a smooth translation of automated techniques into clinical routine.
%In recent years, driven by the release of the extensive Dynamic EchoNet echocardiography dataset (~\cite{ouyang2020video}), there has been an increased adoption of deep learning models aimed at predicting EF and delineating the LV contour. Several innovative architectures have been introduced, including segmentation models (e.g., ~\cite{ouyang2020video,Weihang2023,Meng2024}), direct video regression approaches (e.g.,~\cite{Ouyang,kazemi2020deep,reynaud2021ultrasound,rand2022miccai}), graph networks and keypoints-based models (e.g., ~\cite{Mokhtari2022miccai,ours2022miccai}), and attention-based models (e.g.,~\cite{Mokhtari2023}) - Their potential is somewhat diminished by a common shortfall: the lack of clinically meaningful explanations for the predicted EF. This gap between technological advancement and clinical applicability underscores a critical need for models that do more than just predict; they must also communicate their findings in a manner that aligns with clinical insight and understanding.
%A pivotal approach to improving the interpretability of EF prediction models involves providing explanations in natural language that detail the specific attributes influencing the model's predictions. This could include, for example, descriptions of increased wall thickness in the interventricular septum (hereafter referred to as a septal bulge), foreshortening, or the dynamics of LV key landmarks. These descriptions aim to bridge the gap between the model's output and the clinical insights required by practitioners, thereby fostering trust in automated diagnostics.Our innovation harnesses the capabilities of Large Language Models (LLMs) to assimilate the estimation of LV geometry and relevant attributes, thereby generating textual explanations that are informative and aligned with clinical practices. This method marks a significant step toward developing an AI assistant capable of engaging with clinical users through human-like language, enhancing the interpretability of EF predictions.
Our paper presents three major contributions to the field of cardiovascular ultrasound analysis and interpretation:
\begin{enumerate}
    \item[(1)]{{\em Novel NLE Model for EF Prediction:} We introduce the first NLE model tailored for EF prediction in cardiovascular ultrasound. This model synergizes the analytical depth of modern LLMs with spatiotemporal analysis of geometric features, setting a new benchmark for accuracy and explainability.}
    \item[(2)]{{\em Self-Instruction Training Method:} We develop a novel training approach for the LLaMA model, utilizing GPT-4 to augment explanation examples. By releasing a dataset of approx. 800 self-instructions, we lay the groundwork for future advancements in training LLMs for echocardiography-related tasks.}
    \item[(3)]{{\em Evaluation Metrics for Explanation Output:} Our research extends into the development and application of evaluation metrics specifically designed for assessing the quality of natural language explanations. We show that our model not only achieves precise EF predictions, but also generates explanations that are clinically relevant in a human-like language.}%, thus facilitating an end-to-end inference process.}
\end{enumerate}




% TODO can we also here compare it to concept based models?


% OLDER:
%  However, for many applications, and particularly in the field of medical imaging, such activation maps cannot help much in explaining the prediction to the end user since they often point to trivial or meaningless image regions. For example, for the prediction of EF, as shown in \cite{Mokhtari2023}, activation maps will trivially point to the LV region in the image, which is clinically correct but not clinically meaningful. For these reasons and to augment the explainability of deep learning models with human-readable text, a recent line of work has proposed generating text explanation that will be added to the predicted model outcome. Such models exploit recent progress in vision-language models as well as language models. This subfield of explainable deep learning models, also called {\em Natural Language Explanations (NLE)}, includes models for generating text explanations based on object class attributes~\cite{hendricks2016generating}, models for associating text explanations with image regions~\cite{hendricks2018grounding}, and models that also involve language models such as GPT2 (e.g., ~\cite{sammani2022nlx,kayser2022explaining}) and GPT3 (e.g., \cite{sammani2023iccvw}). 

% % \todo{There is a newer paper on this \cite{sammani2023iccvw}, interestingly they also  report the standard metrics}
% % \todo{Can our approach be compared to other NLE approaches that unify the prediction and explanation task?}
% %NLE models were also very recently introduced to the field of medical imaging (e.g., \cite{kayser2022explaining}), where medical datasets such as Chest X-Ray were augmented with annotations that fit learning of text explanation.  

% Our work is inspired by attribute-based NLE (e.g., ~\cite{hendricks2016generating,hendricks2018grounding}), where text is generated given a list of pre-defined attributes that are detected together with the visual object. 
% In our work, we follow a similar paradigm of explanation that is generated from attributes, albeit the attributes are computed from the predicted geometry of the LV over a full cardiac cycle (hence, spatio-temporal attributes). Our work is also inspired by the more recent NLE models that include pre-trained Large Language Models (LLMs)~\cite{sammani2022nlx,kayser2022explaining}. We explore different model architectures, such as a pre-trained GPT-2 model~\cite{radford2019language} as the final stage of the prediction pipeline to create a smooth and coherent explanation text, which is also partially based on medical knowledge that was inserted into the model during pre-training. 


% PAST WORK related to keypoint-based segmentation in medical -- Integrated:
% \todo{Sarina - There seems to be several applications for contour-based GCN segmentation: similar to our echocardiography challenge, but from a different perceptive (natural objects and chest-Xray}

% S. Zorzi, S. Bazrafkan, S. Habenschuss, and F. Fraundorfer, “Polyworld: Polygonal building extraction with graph neural networks in satellite im- ages,” in IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2022, pp. 1848–1857
% \todo{This one is definetely an interesting one but I think not too related because it builds the graph edges vom already detected keypoints, not based on learned shape priors.}
 
% N. Gaggion, L. Mansilla, C. Mosquera, D. H. Milone, and E. Ferrante, “Improving anatomical plausibility in medical image segmentation via hybrid graph neural networks: applications to chest x-ray analysis,” IEEE Transactions on Medical Imaging, vol. 42, no. 2, pp. 546–556, 2022.

% K. M. Bransby, G. G. Slabaugh, C. Bourantas, and Q. Zhang, “Joint dense-point representation for contour-aware graph segmenta-tion,” in Medical Image Computing and Computer Assisted Intervention– MICCAI: Proceedings, Part III, vol. 14222. Springer, 2023, pp. 519– 528.
% \todo{Those two papers focus on combining segmentation and contours (they even started before our first miccai submission). It is related to Gilles work}
 

% J. Gao, Z. Wang, J. Xuan, and S. Fidler, “Beyond fixed grid: Learning geometric image representation with a deformable grid,” in Computer Vision–ECCV 2020: Proceedings, Part IX 16. Springer, 2020, pp. 108– 125.

% H. Ling, J. Gao, A. Kar, W. Chen, and S. Fidler, “Fast interactive object annotation with curve-gcn,” in IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2019, pp. 5257–5266.
 


% EF AND ECHONET REF: -- INTEGRATED
% \todo{This is from recent SOTA EF prediction / segmentation on Echonet }
% \cite{Weihang2023} is using segmentation masks as cyclical semi-supervision to enhance EF prediction.
% \cite{Meng2024} weakly supervised EF prediction with segmentation labels.
% \cite{Saeed2022} applies contrastive pre-training to improve LV segmentation.
% \cite{rand2022miccai} outperform previous direct EF regression with below 4.0 MAE by using ViT backbone (modified UniFormer)
% \cite{Chen2022} SOTA EF from ISBI 2022
% \cite{Mokhtari2023} transformer based approach that outperforms previous work on EF prediction and simultaneously provides explainability maps. In case of EF regression, they show that the attention maps focus on the LV contour which is clinically correct but not meaningful as a different EF value does not lead to a different attentionmap. 
% \cite{Zeng2023ultrasonic} predict segmentation and EF and keyframes  simultaneously but get worse EF prediction (good segmentation)



% OLD

%\subsubsection{Clinical motivation.}
%\label{sec:clinical_motivation}
% Clearly explaining the reasons for a clinical measurement prediction can be as important as the prediction itself. In particular, in the case of ejection fraction (EF) estimation, an explanation that aligns with the intuition of cardiologists can contribute significantly to their trust. Pathological EF typically has several causes that can be directly referred to visual scans of the left ventricle (LV) on echocardiography images. Providing explanations based on these visual cues can help increase trust and reduce manual "adjustment" time that is often required for automatic methods to be integrated in the clinical diagnosis and treatment. 

% In the past two years, a line of deep learning models has emerged to predict EF, as well as LV shape from echocardiograpy scans~\cite{reynaud2021ultrasound,Mokhtari2022miccai,rand2022miccai,ours2022miccai}, mostly since the introduction of a large public echocardiography dataset (The Dynamic EchoNet~\cite{ouyang2020video}). However, while previous work has introduced several interesting architectures for this task (e.g., segmentation models~\cite{ouyang2020video}, direct video regression~\cite{Ouyang,kazemi2020deep,reynaud2021ultrasound,rand2022miccai}, Graph-Neural Networks~\cite{Mokhtari2022miccai,ours2022miccai}, and keypoints-based models~\cite{ours2022miccai}, \todo{Sarina - are there more approaches from 2023?}), they do not provide explanations on the EF outcome %beyond the LV shape 
% that have a clinical meaning. 



%\subsubsection{Natural language explanation for EF prediction.}
%\label{sec:intro_nle}
% Perhaps a suitable way to explain the EF prediction output is by mentioning, in natural text, attributes that may lead the model to return the prediction. Such text could include e.g. a sentence about the existence and appearance of an increased wall thickness on the interventricular septum (further referred as septal bulge), about foreshortening during the echo scanning, or a text describing the movement of the apex and basal points of the LV. All of this could potentially be used to describe the attributes that lead the model to return a certain prediction. Our model is using training of Large Language Models (LLMs) to integrate estimation of LV geometry and attributes from which such a text explanation can be provided. The final output is then natural human language explaining the EF prediction, a first step towards an AI assistant that can interact with a clinical use in human language. 

% To conclude, the contribution of this paper is three-fold: 
% \begin{enumerate}
%     \item[(1)]{We propose the first NLE model in cardiovascular ultrasound, and specifically for predicting EF. Our model is integrating modern LLMs together with spatiotemporal analysis of visual an geometric features.}
%     \item[(2)]{We provide a self-instruction training method for the LLaMA model, which is based on augmentation of explanation examples by the GPT4 model. We release our set of ~800 self-instruction examples for future training of LLMs on echocargiography tasks.}
%     \item[(3)]{We investigate evaluation metrics for the explanation output, and we show that our model can ultimately provide an end-to-end inference with good EF prediction, as well as good natural text explanation.}
% \end{enumerate}


==> sections/method.tex <==
% openning
Our approach introduces a streamlined pipeline that enriches a GCN-based EF prediction with clinically meaningful explanations. With echocardiography videos as input, a video encoder extracts feature representations, then fed to a spatio-temporal Graph Convolutional Network (GCN) which identifies anatomical keypoints. From these keypoints, the EF is predicted along with geometrical attributes essential for our text generator model, which produces natural language explanations of the EF predictions. An overview is shown in Fig.~\ref{fig:overview}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/miccai_2024_nle.png}
    \caption{\textbf{Overview of the proposed pipeline}
    A US video is fed into a CNN video encoder that outputs a feature representation. The features are passed to a spatio-temporal GCN that returns keypoints for ED and ES. The keypoints serve as 1) input for MLPs that regress the LV volumes \textcolor{green}{(in green)} or the EF directly  \textcolor{orange}{(in orange)} and 2) computation of geometrical attributes that are converted into text snippets that can be parsed into an LLM. The LLM provides a human-like explanation for the EF.} 
    \label{fig:overview}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GCN Model for EF Prediction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-frame GCN Model for EF Prediction in a Single Pass}
\label{sec:gcn_model}

Central to our pipeline is the multi-frame Graph Convolutional Network (GCN) model, engineered to perform EF prediction and contour detection in a single integrated operation. Previous work \cite{ours2022miccai} designed a multi-task multi-frame model that derived the EF value directly from the input encoder. That approach resulted in EF and keypoints prediction being disentangled and less interpretable. Since manual EF computation relies solely on the contours, we modified the architecture to ensure that EF prediction follows the mathematical concept of the ratio between both keypoints volumes. By adding two volume regressors and then fusing the results, we base the model on prior knowledge about the dynamics rather than relying purely on black box predictions. We explored different levels of adding prior knowledge, either by directly regressing the EF from keypoints versus having two separate volume regression branches. 

%This model leverages the spatio-temporal relationships inherent in echocardiography sequences, capturing the dynamic movements and deformations of the heart's structures over time. By processing multiple frames simultaneously, the GCN model effectively maps the evolution of key anatomical points throughout the cardiac cycle, facilitating a nuanced understanding of cardiac function and EF. 
% \todo{I removed more sentences since the did not talk about the method but rather about meta stuff. it now contains all the additions under the assumption that we can show that with numbers in table 1. I am currently revising the models and try to rerun all of them for next week.}

% Integration of spatial and temporal data allows for a more comprehensive analysis than traditional frame-by-frame approaches, leading to a significant improvement in prediction accuracy and efficiency. This subsection will elucidate the architectural nuances of the multi-frame GCN model, emphasizing its role in streamlining EF prediction while maintaining high fidelity to the physiological processes it seeks to model.\todo{To which subsection is it referring to?}


%The proposed model includes three stages: (i) a video encoder that is operating on a sequence of ultrasound frames taken from a full cardiac cycle scan. (ii) a graph convolutional neural network (GCN) that computes keypoints of the LV contours for the full sequence of input frames. (iii) a text explainer module that involves computation of spatio-temporal attributes from the LV contours, and a language model that converts these attributes into a final coherent text explanation to the EF. The contribution of this paper is mostly in stages (ii) and (iii). An overview of our model is in Fig.~\ref{fig:overview}.

% This work builds upon prior research on graph convolutional neural networks \cite{ours2022miccai}. In the following, we will provide a concise overview of the previous work and a detailed description of the modifications to the network. The modified architecture is utilized to generate predictions, and these predictions are used to compute specific attributes that are subsequently used as input for a text generator.

%\subsection{Building blocks}
%\label{subsec:BuildingBlocks}
%Our method consists of four components: a CNN encoder that outputs a feature vector, a decoding graph that regresses the keypoints based on the feature representations, a regression layers that outputs a value for the ejection fraction and a language model that converts the ejection fraction along with attributes derived from the keypoints to a human-readable explanation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Attribute generation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Attribute generation}
\label{subsec:methods:attributeclassifier}

% In clinical routine, ejection fraction is computed based on either manual or semi-automatic annotated contours of the LV endocardium, which can be automatically predicted with the described method. This naturally implies that the shape of the contour is one of the factor that leading to the result values. Some variations in shape can be directly linked to pathological structural changes. Furthermore, temporal deviations from the normal movement can be linked to differences in the EF. For all these, we have designed a set of geometrical processing routines computed from the contour points  
% %,as well as small DNN modules, that operate on the contour points from all frames, and can compute attributes 
% that aim to capture cardiologists intuition when they estimate and assess the EF. This set of attributes was acquired based on clinical feedback from cardiologists. In this section, we present the attributes and the methods to compute them. 
% %\todo{Rewrite depending on whether we add classifiers for the attributes -- we should try to add at least one classifier}

Beyond automatically predicting LV contours, our model also derives attributes that reflect structural changes and temporal deviations due to pathology or acquisition which affect the EF values. Based on clinical insights, we developed geometrical processing routines to compute attributes from LV contour points, capturing the intuition of cardiologists in EF assessment. This section outlines the attributes, grounded in clinical feedback, along with the computation.

\noindent\textbf{Septal bulge:} A septal bulge can be a morphological sign for early hypertensive heart disease \cite{Gaudron2016} and is an asymmetric, localized thickening of the basal-to-mid part of the inter-ventricular septum. It could be detected by calculating a wall thickness ratio over 1.4\cite{marciniak2021septal}. We compute a bulge using the LV convexity which is the distance between a convex hull and the true contour. Ground truth contours were visually inspected while three manual thresholds were set to distinguish prominent bulges from undetected convexity calculated using OpenCV \footnote{www.opencv.org}.

%we calculate contour convexity as the maximum distance between the convex hull and the actual contour. Ground truth contours were visually inspected, and three manual thresholds were set to distinguish prominent bulges from undetected convexity based on convex distance.

%To create artificial bulges, we can use Bezier curves tangential to the lateral contour with orthogonal control points of different realistic sizes
\noindent\textbf{Segment motion:}
The 17-segment model\cite{american2002standardized} is widely used for regional wall motion analysis in multiple views. To simplify the process for 4CH-view, we divide the contour into 7 distinctive segments and calculate the segment movement direction relative to the overall motion as well as the vertical basal movement.

%\todo{not sure whether it can be used}
\noindent\textbf{Apex movement:} Foreshortening is a common problem in 2D echocardiography which results in underestimating the LV volume and inaccurate EF estimation. A foreshortened apex translates throughout the cycle, whereas a true apex almost remains at the same point. Following the approach of \cite{Smistad2020}, we compute the apex movement in the direction of the LV long axis. Based on the distribution in the dataset we set a threshold to indicate suspicious apex movement.

\noindent\textbf{Length-width ratio: }
A normal LV has a bullet-like shape. Cardiovascular diseases such as hypertension or heart failure may change the LV shape despite age and gender being also effecting factors. We decided to use the length-width ratio as a shape measure which is computed by dividing the apex-basal distance by the horizontal mid-septal distance. The length-width ratio is typically around \textbf{2}, as observed during our experiments, while in cases with dilated LV, resulting in a reduced length-width ratio.


%and the thresholds were again chosen based on the distribution in the training dataset.


\noindent\textbf{Sector intersection:} One important requirement for manual and automatic EF computation is to ensure full visibility of the LV within the ultrasound sector.  Therefore, we calculate the ratio of the intersection with the detected LV contours as a quality metric for the EF computation.

\noindent\textbf{Image quality:} 
Image quality will affect the visibility of the LV contours and the wall movement which influences the EF estimation.   %as most image quality research focuses on raw ultrasound beam data, 
We calculate the intensity difference between the LV cavity and the myocardial wall as a measure of their contrast. A higher contrast indicates an improved visibility. However, this metric, though practical, does not cover all dimensions of image quality.

%\subsubsection{EF:} The EF naturally is the most important attribute in this work.

All of the aforementioned attributes are clustered based on their distribution in the annotated dataset. Thresholds were defined for each attribute to create text templates that could be fed into a language model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generation of text explanations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generation of text explanations}
\label{subsec:methods:explanationgeneration}

The ability to translate complex geometrical and spatiotemporal attributes into understandable natural language explanations is critical to bridge the gap between advanced echocardiographic analysis and clinical practice. Our approach encompasses two primary phases: (1) converting the attributes into basic text sentences that describe the underlying clinical observations, and (2) refining these basic sentences into coherent natural language explanations suitable for clinical use, leveraging the capabilities of a Large Language Model (LLM).

{\bf From attribute values to LLM inputs. }
Computed attributes are numerical values that need to be converted into text tokens digestable for the LLM. The first phase involves translating the list of visual and geometric attributes into \textbf{basic sentences} by using thresholds. For instance, the numerical value \textit{bulge}$=500$ is translated to "A bulge value of 500 means that there is no bulge". 
% \todo{we need to distinguish here between LLM input and pseudo explanation}

{\bf Natural Language Refinement with LLM. }
In the second phase, we employ the LLaMA model~\cite{touvron2023llama}, a LLM variant, and train it for generating medical text specifically. We fine-tune LlaMA on a dataset with clinical explanations to ensure that the generated text aligns with clinical terminology and reasoning. To solve the limited availability of expert-generated explanations, we further implement some data augmentation strategies to enrich the training dataset.
% \todo{Chain of though papers https://github.com/Timothyxxx/Chain-of-ThoughtsPapers}

{\bf Synthetic Explanations. } 
By adding prior clinical knowledge, we build more elaborated sentences from the basic sentences as synthetic expert explanations. These sentences articulate the clinical significance of each attribute in a structured format. For instance, an attribute indicating a significant septal bulge would be converted into a more elaborated sentence like "There is a large septal bulge, which may adversely affect the EF."

{\bf Data Augmentation through Self-instruction.}
We adopted a self-\\instruction method~\cite{wang2022self} using the GPT-4 model to augment a small initial dataset containing experts explanations. By feeding 5 expert explanations into GPT-4, along with a chain-of-thought prompt~\cite{Wei2022ChainOT} that includes examples of the input (basic sentences) and the desired output (expert explanation), we instruct GPT-4 to simulate medical expert explanations for novel sets of basic text. This use of chain-of-thought processing with GPT-4 effectively enlarges  our dataset towards a ten times expansion of the initial set.

This dual process ensures that our model not only accurately identifies the visual and geometrical attributes indicative of specific cardiac conditions, but also communicates findings in a way that clinicians can immediately interpret. 
%Integration of LLaMA with the pseudo explanations and augmented dataset positions our methodology at the forefront of interpretability in cardiac imaging, offering useful support for clinical decision making.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% novel metric
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A novel metric to evaluate the EF explanation via LLMs}
\label{subsec:methods:metric_ef_text}
Evaluating unstructured text is crucial to identify errors in clinical LLM, yet human evaluation is time consuming and potentially subjective, highlighting the need for automated metrics. However, initial experiments indicated that even simple adversarial examples could deceive most of the existing metrics for sentence similarity. Given that the output of the proposed LLMs is unstructured text focused on key attributes, we designed a metric specifically aimed at assessing factual correctness. To accomplish this, we use the recently released Mistral model~\cite{jiang2023mistral}, 
%which outperforms previous LLaMA versions and 
another and faster LLM variant.
%offers a speed-up through sliding window attention. 
By creating nine targeted prompts with instructions and one-shot context for Mistral, we evaluate whether attributes are positive (pathological), negative (normal), or unspecified. This approach allows a comparison between ground truth and prediction beyond mere textual similarity. In cases where an attribute is unspecified, its status is considered normal. We quantify the performance by reporting the accuracy, the count of true contradictions, hallucinations, and of missing attributes.%https://huggingface.co/docs/transformers/main/model_doc/mistral
% All of the aforementioned attributes are clustered based on their natural distribution. For this purpose, the trained single frame model from~\cite{ours2022miccai} was used to ran over a large proportion of the training data to compute attributes and examine the distributions. Thresholds were defined for each attribute to create text templates that could be fed into a language model.
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.8\textwidth]{attributes_distribution.png}
%    \caption{Distribution of attributes computed on the single frame model \cite{ours2022miccai} on the EchoNet training data: Length/width ratio, apex movement, bulge/convexity and EF} 
%    \label{fig:distribution}
%\end{figure}
%During inference, attribute scores are computed and compared to the thresholds that set up before. Initial set of text fragments is generated, a text fragment for each attribute, based on text templates. For example, if the bulge attribute score is high, a text template mentioning a large bulge would be added to the initial set, e.g., "The convexity of the septal bulge is large". For this stage we prepared 10 different templates (for all attributes) based on feedback from clinical experts. The initial set of text fragments is then fed to a pretrained GPT2 model to create a smooth and coherent text explanation that connects all fragments, where text gaps are filled with clinincal terms that were learned by the GPT2 during pretraining. 
















% OLD

\begin{comment}
\subsection{Pseudo explanations}
\label{subsec:pseudo}
Based on predefined thresholds for each attribute, we generated a synthetic text. For each attribute and each threshold we randomly select from text snippets. This way the synthetic sample includes all computed attributes in an human readable form.

\subsection{GPT-2}
\label{subsec:gpt2}
We could include it but we know that it underperforms
\begin{enumerate}
    \item GPT2\_real
   \item GPT2\_real\_plus\_synth (not yet trained)
\end{enumerate}

\subsection{Llama2 ? }
Do we want to get another model?
\label{subsec:gpt2}
\begin{enumerate}
    \item ?
\end{enumerate}

\subsection{GPT4-based}
\label{subsec:gpt4}
\begin{enumerate}
    \item GPT4\_CoT\_real
   \item GPT4\_CoT\_real\_plus\_intro
   \item GPT4\_CoT\_real\_plus\_synth
   \item GPT4\_CoT\_real\_plus\_synth\_plus\_intro
\end{enumerate}

\subsection{Llama1 LORA} 
\label{subsec:llama}
\begin{enumerate}
    \item LORA 7B real plus synth
    \item LORA 13B real plus synth
    \item LORA self instruct GPT4 plus CoT
\end{enumerate}


\subsection{Thoughts on EchoClip}
Could be also used to get the attributes? By using the vocab or our attribute sentences? Probably underperforms on EchoNet downsampled data but 
maybe still an interesting thing?
--> Checked for bulge but there is no in the report vocab only sigmoid septum




\subsection{Multi-frame GCN model for EF prediction in single pass}
\label{subsec:methods:gcn}

\todo{How to integrate previous work here? So far we used gt annotations}


\subsection{Generation of text explanations}
\label{subsec:methods:explanationgeneration}
%All of the aforementioned attributes are clustered based on their natural distribution. For this purpose, the trained single frame model from~\cite{ours2022miccai} was used to ran over a large proportion of the training data to compute attributes and examine the distributions. Thresholds were defined for each attribute to create text templates that could be fed into a language model.
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.8\textwidth]{attributes_distribution.png}
%    \caption{Distribution of attributes computed on the single frame model \cite{ours2022miccai} on the EchoNet training data: Length/width ratio, apex movement, bulge/convexity and EF} 
%    \label{fig:distribution}
%\end{figure}
%During inference, attribute scores are computed and compared to the thresholds that set up before. Initial set of text fragments is generated, a text fragment for each attribute, based on text templates. For example, if the bulge attribute score is high, a text template mentioning a large bulge would be added to the initial set, e.g., "The convexity of the septal bulge is large". For this stage we prepared 10 different templates (for all attributes) based on feedback from clinical experts. The initial set of text fragments is then fed to a pretrained GPT2 model to create a smooth and coherent text explanation that connects all fragments, where text gaps are filled with clinincal terms that were learned by the GPT2 during pretraining. 




\end{comment}

==> tables/table_ef.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% \hline
% Model &  frames & Dice (\%)  & MKE (\%)  & EF & mode& explainable \\ \midrule
% \hline
% EchoGraphs\cite{ours2022miccai}  &  1 & $92.1 \pm 3.8$ & $2.2\pm0.9$  &-  & single & no  \\
% EchoNet\cite{Ouyang}  &  1  & $91.7 \pm 4.2$ & $2.5\pm1.2$  & 4.22  & single/single cycle  &  no \\
% \hline
% Transformer\cite{reynaud2021ultrasound}  & 128  & -  & - & 5.32  & single cycle & no  \\
% %EchoGNN\cite{Mokhtari2022miccai}  & ? & 16  & - & $2.3\pm1.0$ & xx  & full cycle &  yes \\
% EchoGraphs\cite{ours2022miccai}  &  16  & $90.3\pm4.3$ & $2.7\pm1.5$  & 4.01  & single cycle & no  \\
% NLE EF (ours)  &  16 & $90.8 \pm4.4$  & $2.5\pm 1.1$   &  4.21  &  single cycle &  yes  \\ 
% \end{tabular}
% \caption{Segmentation and EF accuracy for different methods evaluated on the EchoNet \cite{Ouyang} test set with 1264 patients and two annotated frames (ED and ES) each. MKE = mean keypoint error (mean L1 error in \%). \todo{Need to be filled with more newer numbers, maybe use other SOTA here. We could add the model that is explainable but does not have kpts from Mokthari. WHich sota to add? Without frame selection}}

% \label{tab:ef}
% \end{table}



\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|l|}
\hline
Model & Frames & Dice (\%) & MKE (px) & EF MAE & Cycle & Explainable \\ \hline
%EchoGraphs\cite{ours2022miccai} & 1 & $92.1 \pm 3.8$ & $2.2\pm0.9$ & - & Single frame & No \\ 
EchoNet~\cite{ouyang2020video} & 32 & $91.7 \pm 4.2$ & $2.5\pm1.2$ & 4.22 & Single & No \\ 
%Transformer\cite{reynaud2021ultrasound} & 128 & - & - & 5.32 & Single cycle & No \\ 
EchoGraphs~\cite{ours2022miccai} & 16 & $90.3\pm4.3$ & $2.7\pm1.5$ & 4.01 & Single & No \\ 
EchoCoTr-S~\cite{rand2022miccai} & 36 & N/A & N/A &3.95  & Multi & No \\
GEMTrans~\cite{Mokhtari2023} & 16  & N/A & N/A &4.15  & Multi & Heatmaps \\
NLE EF GCN (Ours) & 16 & $91.5\pm4.3$  & $2.4\pm1.1$ & 4.00 & Single & Text \\
NLE Vol GCN (Ours) & 16 & $91.4\pm4.4$ & $2.4\pm 1.1$ & 4.05 & Single & Text \\ 
%NLE EF GCN Const (Ours) & 16 & $89.3\pm4.8$  & $2.7\pm1.1$& 3.95 & Single cycle & Yes \\ \hline
\hline
\end{tabular}%
}
\caption{Segmentation and EF accuracy for different methods evaluated on EchoNet testset (n=1264) and annotated ED and ES frames (MKE = mean L1 keypoint pixel error). \textit{Multi} refers to whole videos whereas \textit{single} refers to one cycle or ED to ES.
}
\label{tab:ef}
\end{table}


==> tables/table_nle.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{@{}lllllllllll@{}}
% \toprule
% \hline
% Model &  BLEU & ROUGE-2 & bert & sbert & biobert & clinicalbert & medsbert & simcse& mistral score & contradictions \\ \midrule
% \hline
% Pseudo explanations & 0.00 & 0.04 & 0.83 & 0.56 & 0.60 & 0.83 & 0.94 & 0.83& 0.75 & 11  \\
% \hline
% GPT2\  real (maybe retrain) & 0 & 0 & 0 & 0& 0&0 &0 & 0 & 0.62 & 13  \\
% \hline
% GPT4& &  & &  & & & &&& \\
% CoT\  real & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% CoT\  real+intro & 0 & 0 & 0 & 0 &0 &0 & 0 & 0 & 0.72 & 2 \\
% CoT\  real+synth & 0 & 0 & 0& 0 & 0& 0 & 0 & 0 & 0.75 & 5 \\
% CoT\  real+synth+intro & 0 & 0& 0 & 0&0 & 0 & 0 & 0 & 0.73 & 1 \\
% \hline
% LORA& &  & &  & & & &&&  \\
% 7B 1 real plus 1 synth & 0.00 & 0.03 & 0.81 & 0.48 & 0.55& 0.81 & 0.93 & 0.81 & 0.63 & 16 \\
% 7B 1 real plus 10 synth & 0.02 & 0.04 & 0.83 & 0.53 & 0.60 & 0.83 & 0.94 & 0.83&  0.61 & 10 \\
% 7B 1 real plus 70 synth & 0.01 & 0.04 & 0.81 &0.49 &0.56 &0.70 & 0.94  & 0.81 & 0.59 & 16 \\
% 7B self instruct GPT4\  CoT & 0.00 &0.03 &0.80 & 0.53 & 0.59 & 0.80 & 0.94 &0.80 & 0.69 &  11\\
% 13B 1 real plus 1 synth & 0.0 & 0.16 &0.79 & 0.41 & 0.52 & 0.79 & 0.92 & 0.79 & 0.54 & 14 \\
% 13B 1 real plus 10 synth & 0.0 &0.33 & 0.81 &0.54 &0.58 & 0.81 &0.94 &0.81 & 0.69 & 14 \\
% 13B 1 real plus 70 synth & 0.0 & 0.04 &0.82 &0.52 &0.59 & 0.82 & 0.93 & 0.82 & 0.72 & 9 \\
% 13B self instruct GPT4\  CoT & 0.00 & 0.02 & 0.80 & 0.56 & 0.58 & 0.80 &0.95 & 0.80 & 0.72 &  9\\
% \hline
% \end{tabular}
% \caption{Different NLE approaches evaluated for classical NLP metrics ROUGE and BLEU and evaluated by sentence and word similarity (BERT) and plausibility and contractions (mistral). \todo{Need to be filled with  numbers. Self instruct still had the 3 dummy examples in them that is why the numbers slighlty change now.}
% }
% \label{tab:nle}
% \end{table}

% Version 1
% \begin{table}[ht]
% \centering
% \caption{Evaluation of different NLE approaches using classical NLP metrics (ROUGE, BLEU), sentence and word similarity (BERT variants), and contradiction handling (Mistral Score). Further refinement and data updates are anticipated.}
% \label{tab:nle}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{BLEU} & \textbf{ROUGE-2} & \textbf{BERT} & \textbf{sBERT} & \textbf{BioBERT} & \textbf{ClinicalBERT} & \textbf{MedsBERT} & \textbf{SimCSE} & \textbf{Mistral Score} & \textbf{Contradictions} \\ \hline
% Pseudo explanations & 0.00 & 0.04 & 0.83 & 0.56 & 0.60 & 0.83 & 0.94 & 0.83 & 0.75 & 11 \\ \hline
% LLaMA 7B 1 real+1 synth & 0.00 & 0.03 & 0.81 & 0.48 & 0.55 & 0.81 & 0.93 & 0.81 & 0.63 & 16 \\ \hline
% LLaMA 7B 1 real+10 synth & 0.02 & 0.04 & 0.83 & 0.53 & 0.60 & 0.83 & 0.94 & 0.83 & 0.61 & 10 \\ \hline
% LLaMA 7B 1 real+70 synth & 0.01 & 0.04 & 0.81 & 0.49 & 0.56 & 0.70 & 0.94 & 0.81 & 0.59 & 16 \\ \hline
% LLaMA 7B self instruct GPT4\  CoT & 0.00 & 0.03 & 0.80 & 0.53 & 0.59 & 0.80 & 0.94 & 0.80 & 0.69 & 11 \\ \hline
% LLaMA 13B 1 real+1 synth & 0.0 & 0.16 & 0.79 & 0.41 & 0.52 & 0.79 & 0.92 & 0.79 & 0.54 & 14 \\ \hline
% LLaMA 13B 1 real+10 synth & 0.0 & 0.33 & 0.81 & 0.54 & 0.58 & 0.81 & 0.94 & 0.81 & 0.69 & 14 \\ \hline
% LLaMA 13B 1 real+70 synth & 0.0 & 0.04 & 0.82 & 0.52 & 0.59 & 0.82 & 0.93 & 0.82 & 0.72 & 9 \\ \hline
% LLaMA 13B self instruct GPT4\  CoT & 0.00 & 0.02 & 0.80 & 0.56 & 0.58 & 0.80 & 0.95 & 0.80 & 0.72 & 9 \\ \hline
% \end{tabular}
% \end{table}
\iffalse
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{B} & \textbf{R} & \textbf{BERT} & \textbf{sBERT} & \textbf{BioB.} & \textbf{ClinB.} & \textbf{MedsB.} & \textbf{SimCSE} & \textbf{Mistral} & \textbf{Contr.} &  \textbf{Ease} &  \textbf{Count} \\ \hline
Pseudo expl. & 0.00 & 0.04 & 0.83 & 0.56 & 0.60 & 0.83 & 0.94 & 0.83 & 0.75 & 11 & 509 & 54.1 \\ \hline
LLaMA 7B 1:1 synth & 0.00 & 0.03 & 0.81 & 0.48 & 0.55 & 0.81 & 0.93 & 0.81 & 0.63 & 16 & 613 & 70.6 \\ \hline
LLaMA 7B 1:10 synth & 0.02 & 0.04 & 0.83 & 0.53 & 0.60 & 0.83 & 0.94 & 0.83 & 0.61 & 10 & 766 & 74.0\\ \hline
LLaMA 7B 1:70 synth & 0.01 & 0.04 & 0.81 & 0.49 & 0.56 & 0.70 & 0.94 & 0.81 & 0.59 & 16 &1023 &76.2 \\ \hline
LLaMA 7B GPT4\  CoT & 0.00 & 0.03 & 0.80 & 0.53 & 0.59 & 0.80 & 0.94 & 0.80 & 0.69 & 11 & 1355 & 36.5\\ \hline
LLaMA 13B 1:1 synth & 0.0 & 0.16 & 0.79 & 0.41 & 0.52 & 0.79 & 0.92 & 0.79 & 0.54 & 14 & 801 & 63.4 \\ \hline
LLaMA 13B 1:10 synth & 0.0 & 0.33 & 0.81 & 0.54 & 0.58 & 0.81 & 0.94 & 0.81 & 0.69 & 14 & 706 & 59.4\\ \hline
LLaMA 13B 1:70 synth & 0.0 & 0.04 & 0.82 & 0.52 & 0.59 & 0.82 & 0.93 & 0.82 & 0.72 & 9 & 596 & 60.4\\ \hline
LLaMA 13B GPT4\  CoT & 0.00 & 0.02 & 0.80 & 0.56 & 0.58 & 0.80 & 0.95 & 0.80 & 0.72 & 9 & 1546 & 35.5 \\ \hline
\end{tabular}
\caption{Evaluation of NLE approaches using NLP metrics, similarity scores, and contradiction handling.
\todo{Need to be filled with  numbers. Self instruct still had the 3 dummy examples in them that is why the numbers slighlty change now.}
}
\label{tab:nle}
\end{table}
\fi
%gt word count $= 720$ gt reading ease $76.4$


\begin{table}[t]
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Model          & mistral acc$\uparrow$& halluc.$\downarrow$ &contradict.$\downarrow$& missing$\downarrow$& cbert$\uparrow$ & msbert$\uparrow$  & Flesch$\downarrow$ \\
\hline
random\footnotemark                &   0.45      &                    &                &             &                    &                &  \\
LLaVA-Med        &  0.67     &        1.49  &     0.87       &               1.49        &           0.92         &     0.95              &  54.92 \\
%ef\_0212\_13B             & 0.72                 & 1.19      & 0.67                        & 1.33           & 0.93                     & 0.94                             & 64.68                        \\
NLE-EF-13B      & 0.77                         & 0.54       & 1.02                  & 1.50           & 0.93                     & 0.96                          & 58.59                        \\
%ef\_0212\_7B              & 0.74                      & 0.71    & 1.08                      & 1.63          & 0.93                     & 0.95                             & 62.76                        \\
NLE-EF-7B       & 0.77                          & 0.65          & 0.67               & 1.44                & 0.94                     & 0.95                    & 57.20                        \\
NLE-EF-13B self-i & 0.77                    & 0.44      & 1.13                    & 1.65                     & 0.91                     & 0.95                    & 30.91                        \\
NLE-EF-7B self-i & 0.80                         & 0.50       & 0.90                & 1.33           & 0.92                     & 0.95                            & 27.42                        \\
%synthetic                 & 0.77                       & 0.63          & 1.02                  & 1.48                  & 0.94                     & 0.96                  & 56.16                       
\hline
\end{tabular}
\caption{Evaluation of the NLE-EF versions on 48 samples from the EchoNet test set using different averaged metrics such as mistral score accuracy, average number of mistral contradictions, hallucinations and missing attributes, cbert score (clinical BERT), msbert score (sentence medsBERT), and Flesch reading ease.
}
\label{tab:nle}
\end{table}
\footnotetext{{Means random answers to the attributes from sec.\ref{subsec:methods:attributeclassifier}} }
